Co-PatcheR: Collaborative Software Patching with Component(s)-specific Small Reasoning Models

Motivated by the success of general-purpose large language models (LLMs) in software patching, recent works started to train specialized patching models. Most works trained one model to handle the end-to-end patching pipeline (including issue localization, patch generation, and patch validation). However, it is hard for a small model to handle all tasks, as different sub-tasks have different workflows and require different expertise. As such, by using a 70 billion model, SOTA methods can only reach up to 41% resolved rate on SWE-bench-Verified. Motivated by the collaborative nature, we propose Co-PatcheR, the first collaborative patching system with small and specialized reasoning models for individual components. Our key technique novelties are the specific task designs and training recipes. First, we train a model for localization and patch generation. Our localization pinpoints the suspicious lines through a two-step procedure, and our generation combines patch generation and critique. We then propose a hybrid patch validation that includes two models for crafting issue-reproducing test cases with and without assertions and judging patch correctness, followed by a majority vote-based patch selection. Through extensive evaluation, we show that Co-PatcheR achieves 46% resolved rate on SWE-bench-Verified with only 3 x 14B models. This makes Co-PatcheR the best patcher with specialized models, requiring the least training resources and the smallest models. We conduct a comprehensive ablation study to validate our recipes, as well as our choice of training data number, model size, and testing-phase scaling strategy.

==> one-per-component/0-abstract.tex <==
\begin{abstract}
Motivated by the success of general‑purpose large language models (LLMs) in software patching, recent works started to train specialized patching models.
Most works trained one model to handle the end‑to‑end patching pipeline (including issue localization, patch generation, and patch validation).
However, it is hard for a small model to handle all tasks, as different sub-tasks have different workflows and require different expertise.  
As such, by using a $70$ billion model, SOTA methods can only reach up to $41$\% resolved rate on \swebenchverified. 
Motivated by the collaborative nature, we propose \sys, the first \emph{collaborative patching system} with small and specialized reasoning models for individual components.
We propose a specific task design and training recipe for each model.
Our localization model pinpoints the vulnerable lines through a two-step procedure, and our generation model combines patch generation and critic.
Our hybrid patch validation first has a custom model for crafting vulnerable test cases and judging patch correctness, followed by a majority vote-based patch selection.
Through extensive evaluation, we show that \sys achieves~\textbf{44\%} resolved rate on \swebenchverified with only 3$\times$14B models
This makes \sys the state-of-the-art (SOTA) open-source patcher with the least training resources and the smallest models.
We conduct a comprehensive ablation study to validate our proposed recipes, as well as our choice of training data number, model size, and testing-phase scaling strategy.
We will release our code and models upon acceptance.  
%~\textcolor{blue}{Robin: Are we releasing our repo during submission? We can have an empty link and eventually add stuff there}
\end{abstract}


==> one-per-component/1-intro.tex <==
\section{Introduction}
\label{sec:intro}

Software patching is a time-intensive and cognitively demanding task, especially for large and complex codebases.
In the real world, effective patching often requires a combination of \textit{complementary skills}: locating the faulty component, generating plausible fixes, and validating the changes. 
Recent approaches leverage general-purpose LLMs~\cite{} to construct patching agents with three components, responsible for localization, generation, and validation, respectively.
They have demonstrated remarkable performance on SOTA benchmarks (e.g., SWE-bench~\cite{}) and show significant potential to reduce developer burden while improving software robustness at scale.

Despite these promising results, concerns about cost efficiency and data privacy have motivated the development of customized patching models. 
Current approaches predominantly train one model for multiple patching components through supervised fine-tuning (SFT) or reinforcement learning.   
Specifically, early works (SWE-SynInfer~\cite{} and SWE-Gym~\cite{}) fine-tuned $72$B and $32$B open-source models through simple supervised data and achieved around $30$\% resolved rates on the SWE-bench-Verified.
More recent methods have implemented rule-based rewards and trained reasoning models with reinforcement learning, with SWE-RL~\cite{} achieving the highest resolve rate of 41\% on SWE-bench-Verified using a $70$B model.
However, this monolithic approach contradicts the real-world patching paradigm, where specialized engineers typically collaborate by \textit{dividing responsibilities according to their expertise}.


Inspired by the collaborative workflow, we propose \sys, the first patching agent with \textit{collaborative small reasoning models designed specifically for individual components}. 
Our key insight for having component-specific models is that each component has its own inputs, outputs, and capability requirements.
For example, the localization component requires the model to interpret the issue description and navigate the codebase without needing to generate code.
For generation, it needs to generate correct patches, but doesn't require creating test cases, which are essential for validation.
Given the non-trivial differences, it is challenging for one small model to handle all these sub-tasks. 
Following this intuition, we craft a tailored training recipe for each component, aiming to~\textit{minimize the model size while preserving performance}.
Specifically, we first train the localization model with a two-step procedure, where the model first identifies the affected files and then pinpoints the specific lines responsible for the issue.
This task decomposition reduces the task complexity and context length, making it more suitable for small models.
For patch generation, we train the generation model to review and refine its generated patches. 
With this self-critical capability, the patch generation model can prevent common errors and generate higher-quality candidates. 
Finally, we train a model to generate multiple and diverse vulnerable test cases (PoC) and judge the patch correctness based on the PoC execution outcomes.
We use this model together with available functionality tests and a majority vote mechanism to select the final patch. 
For all three models, we apply model distillation with a novel data construction method to enable their reasoning capabilities.
Different from existing distillation models (e.g., Sky-T1~\cite{sky_t1_2025}), we find that~\textit{creating reasoning data with correct answers is critical for our fine-tuned model to achieve high performance}. 

Through extensive experiments, we first show that when using only~\textbf{3$\times$14B} models, \sys can achieve a~\textbf{XXX\%} resolved rate on \swebenchverified with XXXX patch candidates. 
Compared to SWE-RL, \sys achieves a high resolved rate with XXX\% fewer parameters and XXX\% fewer samples. 
Besides, \sys only needs to run one 14B model at a time, which is much more efficient than SOTA methods during the testing phase.
Furthermore, with our specific reasoning data construction method, \sys only requires 2K data for training, which is much more efficient than SOTA methods (at least 30K).
We then conduct a comprehensive ablation study for each component to validate its task design and training recipe.
% Our ablation study also compares our models with SOTA commercial models and demonstrates that with\TODO{AX} more samples, our models can beat leading commercial models with\TODO{AX} more parameters on each component. 
Finally, we validate the necessity of testing-phase reasoning, as well as our choice of data number and model size, through more ablation studies. 
We also find that long reasoning is not very helpful for our task. 

\textbf{Contributions.}
We propose \sys, the first collaborative patching system with component-specific reasoning models. 
\sys is the most data- and parameter-efficient patcher that offers greater effectiveness, efficiency, and modularity than existing patchers with customized models.
\sys ranks among the top-10 on \swebenchverified, outperforming most patchers with commercial models. 
We propose specific training recipes for each model and obtain some new findings that are unique to patching (Section~\ref{sec:eval}).
%but conflict with previous observations on the general tasks.


==> one-per-component/3-tec.tex <==
\section{Key Technique}
\label{sec:tech}

\subsection{Overview}
\label{sec:tech_overview}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\textwidth]{figs/co-patcher_plot.pdf}
\caption{The overall training pipeline of \sys.}
\label{fig: overall}
\vspace{-.2in}
\end{figure*}

\textbf{Problem setup.}
We target the software patching problem, where we are given a software repository with one or multiple issues/bugs.
Each issue has a simple text description, which may contain additional information such as desired behaviors and vulnerable inputs. 
Each issue may affect one or more functions in the repository.
The task aims to automatically analyze the issue and generate patches that fix all affected functions while preserving the behaviors of the unaffected functions.
This is typically evaluated by running the hidden testing cases crafted by the repository developers. Here is an example in Appendix~\ref{XX}.
% \textcolor{blue}{Robin: We need an illustrative example for this}

\textbf{Technical insight.}
As discussed in Section~\ref{sec:rw}, solving the patching problem automatically requires building an agent system with multiple components, where each component has one or multiple LLM ``brain(s)'' and a set of tools (can also be treated as a sub-agent).
Most existing LLM-based agentic systems for patching use the general-purpose LLMs as the brains (e.g., OpenAI o3/o4, Anthropic Claude), which are large in size and computationally costly. 
Most recently, there have been some early works on training specialized small models to replace the general LLMs, but their model sizes are still relatively large, while, more importantly, their performances are limited.

In this paper, we argue that designing specialized, separate small models is essential for program-patching.
First, developing small and task-specific agents improves the overall efficiency of the patching system. 
This approach avoids the redundant capacity of general-purpose LLMs and may outperform them in specific capabilities.
For instance, a program patching system does not need to process images or video; instead, it must precisely understand the repository, reason about issues, and generate correct fixes.
Second, as demonstrated in Table~\ref{tab:diff}, components of a patching system differ significantly in task type, input-output format, and more importantly, the required model capabilities.
Localization and generation are generative tasks, while validation is a discriminative task requiring a critique model.
The localization component must develop a comprehensive yet coarse-grained understanding of the repository structure.
It must interpret the issue description and efficiently identify relevant code based on semantic relationships.
In contrast, the generation component focuses on fine-grained reasoning about local code chunks and requires stronger generative capabilities to propose patching solutions.
The validation component also examines local code, but primarily needs critical evaluation abilities to assess patch correctness.
This hypothesis is supported by existing works~\cite{wei2025swe,xie2025swe} that trained large models (>70B) using various methods (SFT, offline RL, online RL) yet achieved relatively low performance.
The experimental results in Section~\ref{sec:eval} also support our claim.
% \textcolor{blue}{Robin: We need explicitly mention some evidence here (e.g., some ablations) to support the argument of specialized model vs. generalized model. Otherwise, only conceptual claims sound a bit week}

Based on these findings, we propose~\emph{to train a small but fine-grained model for each component and use them together in the agent system}.
Our approach allocates parameters more efficiently by focusing each model on mastering a specific capability set rather than diluting learning across disparate tasks.
We demonstrate that component-specific models (7B-14B) achieve superior performance because the capabilities required for individual components align more precisely with the specific requirements outlined in Table~\ref{tab:diff}.
% In this paper, we argue that specialized models are essential for program-patching. 
% First, having small and task-specific models improves an agent’s overall efficiency.
% More importantly, this strategy avoids the waste of the redundancy capacity of general-purpose LLMs, and the specialized models may outperform general-purpose LLMs in some specific capabilities. 
% Specifically,  
% Our goal, therefore, is to develop an effective training paradigm for small models for patching that focuses on learning patching-specific capabilities, achieving a better balance between effectiveness and efficiency.

\input{tables/components-compare}

% Different from most existing works that train a model for the entire pipeline, we propose to~\emph{design more fine-grained and specialized models for different components}. 
% Our key insight is that each component in the agent pipeline is different in terms of the task type, the input and output format, and, more importantly, the model capabilities.
% We specify the differences in Table~\ref{tab:diff}.
% First, both localization and generation are generative tasks, and validation is a discriminative task that requires a critique model.
% Besides, all three components have their unique inputs and tool sets. 
% More importantly, these components require different model capabilities from three aspects. 
% As localization's job is to find the code chunks related to the issue, the corresponding model needs to first have a comprehensive but coarse-grained understanding of the repository.
% It is also required to understand the issue and quickly search the related code based on keywords or key semantics.  
% Generation model, on the other hand, does not require understanding the overall repository structure, however, it requires a more fine-grained reasoning of local code chunks, and it needs stronger generative capability to propose patching solutions.
% A model in validation also mainly focuses on local code chunks, but instead of proposing solutions, it should have a strong critical capability to judge the patches' correctness. 
% Note that model capability is a vague concept; we instantiate it from two aspects, but we do not claim these are the only aspects. \textcolor{blue}{Robin: We need explicitly mention some evidence here (e.g., some ablations) to support the argument of specialized model vs. generalized model. Otherwise, only conceptual claims sound a bit week}

% Based on the non-trivial differences across different components, we argue that it may be challenging for~\emph{one small model} to learn to digest very different tasks and learn the diverse capabilities at the same time.
% This hypothesis has been validated by existing works that train a fairly large model (70B to 96B) with different methods (SFT, offline RL, online RL) but still achieve a relatively low performance. 
% On the contrary, given the uniqueness of these components, it is a natural idea~\emph{to train a small but fine-grained model for each component and use them together in the agent system}.
% This is also aligned with our main claim that patching requires specialized models.
% Rather than having an agent-specific model, we push the specification to another level and propose to train component-specific models.  
% Here, we envision that each component-specific model can have an even smaller size (7B or 14B) as the capabilities required for each model are less complex and can learn component-specific capabilities listed in Table~\ref{tab:diff}. 

\textbf{Technical challenges and high-level design.}
The high-level challenge for realizing our vision is to~\emph{reduce each component’s model to the smallest feasible size without sacrificing too much performance}.
More concretely, we need to first design a~\emph{data-efficient} training recipe for each component-specific model (Challenge \ding{182}).
Once we have the models, we also need to decide how to effectively integrate them into the overall agent system (Challenge \ding{183}).  

\underline{Solve challenge \ding{182}.}
In general, we propose to train a reasoning model for each component, as each sub-task requires reasoning capabilities.
As shown in Section~\ref{sec:eval}, training reasoning models can achieve a better performance than training non-reasoning models even with fewer training samples, making the model training even more data- and cost-efficient.  
To obtain such a reasoning model, we propose to distill a large reasoning model with supervised fine-tuning.
Recent research has shown that high-quality distillation data enables training effective small reasoning models for math and coding tasks with limited computational resources~\cite{sky_t1_2025,muennighoff2025s1}. 
In contrast, training reasoning models with reinforcement learning requires substantially more samples and computational power, contradicting our efficiency goals. 
Additionally, without well-designed intermediate process rewards, training based solely on outcome rewards becomes costly and unstable~\cite{pan2024training}.
Later we detail our specific recipe for each component, including data collection, task design, and distillation of data generation and filtering.
Here, we highlight some key novel designs.
For localization, we divide the task into two lower-complexity sub-tasks, generate training data separately, and mix the data for model training.
The trained model can perform both tasks, where each task has a lower complexity (and is more suitable for small models).
For generations, we integrate ``critic training data'' where the model reviews its own code in subsequent dialogue turns, enabling better reasoning about patching errors.
For validation, we train the model to (1) generate Proofs of Concept (PoCs) that trigger the target issue and (2) evaluate patch correctness based on issue descriptions and PoC execution outcomes.
This extra PoC generation and execution provide necessary dynamic information for deciding the patch correctness.

\underline{Solve challenge \ding{183}.}
We adopt PatchPilot's~\cite{li2025patchpilot} cost-efficient agent architecture as our system scaffold.
As shown in Table~\ref{tab:diff}, our localization component follows a pre-defined workflow to output potential buggy code chunks related to the target issues.
The generation component then generates patch candidates that modify the identified chunks.
As shown in Section~\ref{sec:eval}, we discover that having our small model generate multiple and diverse candidates can improve the overall performance of the agent. 
This can be considered a form of testing phase scaling. 
Note that we no longer ask the model to generate a patch plan, as we observe that it is already included in the generation model's reasoning process. 
For validation, we implement a two-stage process: first, a model-based security check where our trained model generates PoCs and evaluates whether patches fix the issue; 
second, a model-free functionality test that runs patches against public functionality tests. We rank patches based on dynamic testing results (including PoC tests and functionality tests) to identify the highest-scoring candidates. 
When multiple patches achieve the same highest score, we apply majority voting based on normalization~\cite{xia2024agentless} to select the final patch.


\subsection{Training Recipe}
Our training recipe consists of three key components: issue selection, data construction, and data filtering. 
Issue selection and data filtering strategies are common across all components, while data construction is tailored to each component's specific requirements. 
This section details our design choices and their rationales.


\subsubsection{Issue Selection}
\label{subsec:issue_selection}
We select training issues and the corresponding repositories from the SWE-bench training set and SWE-Gym dataset, which contains \textit{different repositories from its test set}. 
Our selection criteria focus on two key factors:
First, we prioritize \emph{diversity} by selecting issues from different repositories across different time periods to improve model generalization. 
Second, we include issues with \emph{varying difficulty levels}, following recent work by S1~\cite{muennighoff2025s1} showing that challenging cases improve reasoning abilities with limited training data. 
We quantify the difficulty using the number of files changed in the fix. For example, simple issues require changing only one file, while difficult issues require changes to five or more files.
As shown in~\ref{sec:eval}, in general, the performance of our models first increases as the training data grows and then remains at a similar level. 
Guided by this trend, we select only~\emph{2,000} training issues, which is significantly fewer than existing RL-based methods, e.g., 11M in SWE-RL~\cite{wei2025swe}. \textcolor{blue}{Robin: since we are using SWE-bench-related data for training, we need to **clearly** explain how we do the deduplication -- give them some evidence that our training data has no data leakage at all, otherwise the reviewers will raise significant concerns.}


\subsubsection{Data construction.}
The data construction process is significantly different for each component as they have different task types and input-output formats.

\textbf{Localization}
The key challenge for localization is to efficiently identify code chunks related to issues while keeping the task manageable for a small model.
When designing the task, we must consider both the limited context length and reduced parameter capacity of smaller models.

Rather than training the model to directly identify issue-related code chunks from the entire repository, we decompose localization into two sequential sub-tasks: file localization and line localization.
File localization identifies issue-related files in the repository structure, while line localization pinpoints the specific code chunks within those files. 
This decomposition offers two key advantages. 
First, it creates simpler sub-tasks better suited to small models' capabilities. 
Second, it provides explicit guidance to the model reasoning process, improving efficiency. 
As shown in Table~\ref{tab:diff}, for file localization, we provide the issue description and repository file structure as input. 
For line localization, we input the issue description and the code from each selected file (splitting files that exceed the model's context limit). 
This design significantly reduces context length for each sub-task and eliminates redundant information, further simplifying the model's reasoning requirements (see Appendix~\ref{XX} for examples with the input prompt).
Finally, we use \claudereasoning~\cite{claude37} to generate distillation data with a reasoning chain.
The reasons for choosing \claudereasoning over other reasoning models are that some models (e.g., OpenAI models) do not provide their reasoning chains.
Among the two main open-source models, DeepSeek-r1~\cite{guo2025deepseek} tends to give overly long reasoning chains, making it easy for our model to learn noisy steps.
QwQ~\cite{qwq32b}, meanwhile, performs poorly on patching-related tasks.

\textbf{Generation}
The key novelty of our generation model is to utilize Critique Fine-Tuning (CFT) for patch generation task.
Unlike standard supervised fine-tuning (SFT), which relies on binary <question, answer> pairs, CFT constructs ternary examples <question, answer, critique>. 
Both the answer and its critique are generated by a teacher model, so the model learns not only to produce an answer but also to diagnose and refine existing ones, thereby acquiring stronger reasoning skills during training. 
Such a process could further deepen the model's understanding of the target issues and potentially yield higher-quality patches.

For both tasks, we design the input prompt as a combination of a task instruction and a format instruction. 
Here, the format instruction specifies the desired format for the generated patches (search and replace), together with a few-shot example.
The task instruction for critique combine the whole conversation of generation task as input to output the critique analysis of the patch whether fix the issue.
Appendix~\ref{} shows concrete examples. 


\textbf{Validation}
The high-level goal of validation is to decide whether a candidate patch fixes the issue (correctness of the patch) and whether it affects other benign functions (correctness of functionality).
For functionality correctness, we can retrieve the public testing cases from each project and run dynamic testing against our patches.
The key is to design the patch-correctness validation. 
To enable dynamic testing, we propose to train the validation model to generate testing inputs that can trigger the target issue (PoC) and make a PoC execution result judgment. 
The generation of PoC and judgement represents a significantly more complex challenge than patch generation, as it necessitates the model's capacity to infer intermediate program states and conditional logic flows accurately.
This design is similar to a hybrid program analysis approach that mixes static with dynamic analysis to balance the soundness, precision, and efficiency~\cite{}.  

Here, we use the same set of training issues as the previous components but use multiple teacher models (including Claude-3.7-sonnet and o4-mini) to collect distillation data to teach the model to generate more diverse and correct PoCs.
For PoC generation, our input prompt contains the issue description and an instruction for the model to generate PoC testing following a certain format.
For poc running correctness judgment, the input is designed as the issue description, the current patch, and its PoC execution output to output whether the patch fix the issue. \textcolor{blue}{Robin: We have LLM as a judge and majority vote, if PoC execution has ties, right?}



\subsection{Data filtering.}
After generating the data, we then consider applying filters based on three aspects: final answer correctness, reasoning length, and reasoning quality. 
First, based on our empirical observation, we decide to filter out the training samples that lead to wrong answers, as training with these noisy samples will hurt  model performance.
This observation does not align with existing work~\cite{sky_t1_2025} where they state that data with wrong answers is still useful for models to learn the reasoning structure in math problems.
Second, we filter out samples with excessively long reasoning chains, as long reasoning offers no benefit to our task. 
Worse yet, such data can even cause model collapse and jeopardize training efficiency.
Finally, we conduct a manual examination of the reasoning chains of difficult issues and remove those with irrational reasoning. 

% Using the data collected, we train our localization model with the objective function in Eqn.~\eqref{eq:loss}.

% \begin{equation}
% \label{eq:loss}
% \mathcal{L}_{\text{SFT}} = -\frac{1}{N}\sum_{i=1}^{N}\sum_{t=1}^{T_i} \log P_\theta(y_{i,t}|y_{i,<t}, x_i)
% \end{equation}



==> tables/components-compare.tex <==
\begin{table}[t]
  \centering
  \caption{The summarization of the differences across three components of a patching system. Desc. denotes descriptions.}
  \label{tab:diff}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{r|c|cc|cc}
      \toprule
      \multirow{2}{*}{\textbf{Components}} 
        & \multirow{2}{*}{\textbf{Task type}} 
          & \multicolumn{2}{c|}{\textbf{Format}} 
            & \multicolumn{2}{c}{\textbf{Capabilities}} \\
      \cmidrule(lr){3-6}
        & 
          & Input             & Output          & Relation scope                     & Specialized capability              \\
      \midrule
      \multirow{2}{*}{Localization}
        & \multirow{2}{*}{Generative}
          & Issue desc. \& file structure  
                           & Candidate files 
                                               & \multirow{2}{*}{\makecell[l]{Global \& local\\Coarse-grained}}
                                               & \multirow{2}{*}{\makecell[l]{Understand repo structure\\Root cause identification}} \\
        & 
          & Issue desc. \& file contents    
                           & Code chunks     &                                     &                                     \\
      \midrule
      \multirow{2}{*}{Generation}
        & \multirow{2}{*}{Generative}
          & Issue desc. \& code chunks         
                           & Issue analysis      
                                               & \multirow{2}{*}{\makecell[l]{Local\\Fine-grained}}
                                               & \multirow{2}{*}{\makecell[l]{Reason about issue \\Generate patches}} \\
        & 
          &   
                           & Patch diff      &                                     &                                     \\
      \midrule
      \multirow{2}{*}{Validation}
        & \multirow{2}{*}{Discriminative}
          & Issue description                
                           & Dynamic test and refine  
                                               & \multirow{2}{*}{\makecell[l]{Local\\Fine-grained}}
                                               & \multirow{2}{*}{\makecell[l]{Test generation and be critical with patches}} \\
        & 
          & Patch candidates        
                           &  Test execution critic
                                               &                                     &                                     \\
      \bottomrule
    \end{tabular}%
  }
\vspace{-0.2in}
\end{table}


==> todo.tex <==
A list of appendix

2. ablation
    2.1 compare long reasoning and short reasoning with claude 

3. ablation-localization
    3.1 data size(500, 1000, 2000, 5000)
    3.2 model size(7b, 14b, 32b)
    3.3 testing-phase scaling
        3.3.1 sample 1,3,5,7 for localization
        3.3.2 for final resolved rate

4. ablation-validation
    4.1 train one model and use different prompts to generate two pocs
    4.2 data size(500, 1000, 2000)
    4.3 model size(7b, 14b, 32b)
    4.4 testing-phase scaling
        4.4.1 samples 1,3,5,7 for poc 
        4.4.2 for final resolved rate

5. hyper-parameters details

6. voting
    6.1 compare majority vote and orm


    


Wishlist for rebuttal

1. Model family, what about llama models??
2. Other agent scaffold. 
3. training curve - shuffle? or lr schedule
4. why we cannot beat large model

